Body Size and Depth Disambiguation in Multi-Person Reconstruction from Single Images

We address the problem of multi-person 3D body pose and shape estimation from a single image. While this problem can be addressed by applying single-person approaches multiple times for the same scene, recent works have shown the advantages of building upon deep architectures that simultaneously reason about all people in the scene in a holistic manner by enforcing, e.g., depth order constraints or minimizing interpenetration among reconstructed bodies. However, existing approaches are still unable to capture the size variability of people caused by the inherent body scale and depth ambiguity. In this work, we tackle this challenge by devising a novel optimization scheme that learns the appropriate body scale and relative camera pose, by enforcing the feet of all people to remain on the ground floor. A thorough evaluation on MuPoTS-3D and 3DPW datasets demonstrates that our approach is able to robustly estimate the body translation and shape of multiple people while retrieving their spatial arrangement, consistently improving current state-of-the-art, especially in scenes with people of very different heights

==> comandosnuevos.tex <==
\newcommand{\comment}[1]{}



\newcommand{\bmath}[1]{\mbox{$\mathbf{#1}$}}

\newcommand{\nrsfm}[0] {{\sc nrs{\rm\em f}\sc m }}
\newcommand{\nrsfmS}[0] {{\sc nrs{\rm\em f}\sc m}}
\newcommand{\sfm}[0] {{\sc s{\rm\em f}\sc m }}
\newcommand{\sfmS}[0] {{\sc s{\rm\em f}\sc m}}
\newcommand{\etals}{\emph{et al.}}
\newcommand{\timescomp}{\hspace{-1mm}\times\hspace{-0.5mm}}
\newcommand{\minuscomp}{\hspace{-1mm}-\hspace{-1mm}}
\newcommand{\edm}{\textrm{edm}}
\newcommand{\dist}{\textrm{dist}}
\newcommand*\rot{\rotatebox{90}}


%lowercase--------------------------------
\newcommand{\bzero}{\textbf{0}}
\newcommand{\bone}{\textbf{1}}
\newcommand{\ba}{\mathbf{a}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\bc}{\mathbf{c}}
\newcommand{\bd}{\mathbf{d}}
\newcommand{\be}{\mathbf{e}}
\newcommand{\bff}{\mathbf{f}}
\newcommand{\bg}{\mathbf{g}}
\newcommand{\bh}{\mathbf{h}}
\newcommand{\bl}{\mathbf{l}}
\newcommand{\bn}{\mathbf{n}}
\newcommand{\bo}{\mathbf{o}}
\newcommand{\bp}{\mathbf{p}}
\newcommand{\bq}{\mathbf{q}}
\newcommand{\br}{\mathbf{r}}
\newcommand{\bs}{\mathbf{s}}
\newcommand{\bts}{\tilde{\mathbf{s}}}
\newcommand{\bt}{\mathbf{t}}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\btu}{\tilde{\mathbf{u}}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\btx}{\tilde{\mathbf{x}}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bz}{\mathbf{z}}

%uppercase--------------------------------
\newcommand{\bA}{\mathbf{A}}
\newcommand{\bB}{\mathbf{B}}
\newcommand{\bC}{\mathbf{C}}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\bF}{\mathbf{F}}
\newcommand{\btF}{\tilde{\mathbf{F}}}
\newcommand{\bG}{\mathbf{G}}
\newcommand{\bH}{\mathbf{H}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bJ}{\mathbf{J}}
\newcommand{\bK}{\mathbf{K}}
\newcommand{\bL}{\mathbf{L}}
\newcommand{\bM}{\mathbf{M}}
\newcommand{\bN}{\mathbf{N}}
\newcommand{\bP}{\mathbf{P}}
\newcommand{\btP}{\tilde{\mathbf{P}}}
\newcommand{\bQ}{\mathbf{Q}}
\newcommand{\bR}{\mathbf{R}}
\newcommand{\btS}{\tilde{\mathbf{S}}}
\newcommand{\bS}{\mathbf{S}}
\newcommand{\bT}{\mathbf{T}}
\newcommand{\btT}{\tilde{\mathbf{T}}}
\newcommand{\bU}{\mathbf{U}}
\newcommand{\bV}{\mathbf{V}}
\newcommand{\bW}{\mathbf{W}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\bY}{\mathbf{Y}}
\newcommand{\bZ}{\mathbf{Z}}

\newcommand{\1}{\bmath{1}}
\newcommand{\0}{\bmath{0}}

%hat--------------------------------
\newcommand{\bhA}{\hat{\mathbf{A}}}
\newcommand{\bhc}{\hat{\mathbf{c}}}
\newcommand{\bhd}{\hat{\mathbf{d}}}
\newcommand{\bhF}{\hat{\mathbf{F}}}
\newcommand{\bhG}{\hat{\mathbf{G}}}
\newcommand{\bhH}{\hat{\mathbf{H}}}
\newcommand{\bhJ}{\hat{\mathbf{J}}}
\newcommand{\bhK}{\hat{\mathbf{K}}}
\newcommand{\bhM}{\hat{\mathbf{M}}}
\newcommand{\bhX}{\hat{\mathbf{X}}}




%mathcal--------------------------------
\newcommand{\mA}{\mathcal{A}}
\newcommand{\mC}{\mathcal{C}}
\newcommand{\mD}{\mathcal{D}}
\newcommand{\mE}{\mathcal{E}}
\newcommand{\mF}{\mathcal{F}}
\newcommand{\mI}{\mathcal{I}}
\newcommand{\mK}{\mathcal{K}}
\newcommand{\mM}{\mathcal{M}}
\newcommand{\mN}{\mathcal{N}}
\newcommand{\mL}{\mathcal{L}}
\newcommand{\mP}{\mathcal{P}}
\newcommand{\mR}{\mathcal{R}}
\newcommand{\mS}{\mathcal{S}}
\newcommand{\mT}{\mathcal{T}}
\newcommand{\mmt}{\mathcal{t}}
\newcommand{\mU}{\mathcal{U}}
\newcommand{\mW}{\mathcal{W}}
\newcommand{\mmx}{\mathcal{x}}
\newcommand{\mZ}{\mathcal{Z}}




%mathbb--------------------------------
\newcommand{\mbR}{\mathbb{R}} %symbol for the Real numbers


%symmbols--------------------------------
\newcommand{\Avvo}{\mathcal{A}}
\newcommand{\Tvvo}{\mathcal{T}}
\newcommand{\balpha}{\boldsymbol{\alpha}}
\newcommand{\bdelta}{\boldsymbol{\delta}}
\newcommand{\bDelta}{\boldsymbol{\Delta}}
\newcommand{\blambda}{\boldsymbol{\lambda}}
\newcommand{\bLambda}{\boldsymbol{\Lambda}}
\newcommand{\bmu}{\boldsymbol{\mu}}
\newcommand{\bgamma}{\boldsymbol{\gamma}}
\newcommand{\bGamma}{\boldsymbol{\Gamma}}
\newcommand{\bSigma}{\boldsymbol{\Sigma}}
\newcommand{\btheta}{\boldsymbol{\theta}}
\newcommand{\bvartheta}{\boldsymbol{\vartheta}}
\newcommand{\bTheta}{\boldsymbol{\Theta}}
\newcommand{\brho}{\boldsymbol{\rho}}
\newcommand{\bphi}{\boldsymbol{\phi}}
\newcommand{\bvarphi}{\boldsymbol{\varphi}}
\newcommand{\bPhi}{\boldsymbol{\Phi}}
\newcommand{\bpsi}{\boldsymbol{\psi}}
\newcommand{\bPsi}{\boldsymbol{\Psi}}
\newcommand{\bxi}{\boldsymbol{\xi}}
\newcommand{\bUpsilon}{\boldsymbol{\Upsilon}}
\newcommand{\bomega}{\boldsymbol{\omega}}
\newcommand{\bOmega}{\boldsymbol{\Omega}}


\newcommand{\mo}{\boldsymbol{o}}

\newcommand{\berror}{\boldsymbol{\varepsilon}}

\newcommand{\st}{{\;t}}
\newcommand{\sk}{{\;k}}
\newcommand{\tms}{\hspace{-1mm}\times{\hspace{-1mm}}}
\newcommand{\hh}{\hspace{-1mm}}



\newcommand{\argmin}{\operatornamewithlimits{arg\,min}}
\newcommand{\argmax}{\operatornamewithlimits{arg\,max}}




\newcommand{\Err}{\textrm{Err}}
\newcommand{\Rot}{\textrm{rot}}
\newcommand{\Trans}{\textrm{trans}}


\renewcommand{\labelitemi}{-}
%\renewcommand{\labelitemii}{\Radioactivity}
%\renewcommand{\labelitemiii}{\Biohazard}


==> figure_supp_coco.tex <==
\begin{figure*}[t]
  \vspace{-0.1cm}
  \includegraphics[width=\linewidth, trim={0.1cm 0.1cm 0cm 0}, clip = true]{figures/coco_supp.png}
        \put(-485,4){{{Input image}}}
        \put(-338,4){{{CRMH~\cite{jiang2020_multiperson}}}}
        \put(-115,4){{{Ours}}}
  \vspace{0.2cm}
  \caption{\small{\textbf{Qualitative results}. We visualize the results of our method from different viewpoints: front (green background), top (blue background), and side (red background) views. We compare the results with CRMH~\cite{jiang2020_multiperson} and improve depth order and overall scene coherence. Note that CRMH does not estimate a plane. We add the same plane estimated by our method for the visualization purposes.
%   We have improved results in terms of depth order and overall scene coherence. Notice people's depth order and sizes.
  %(see Eq.~\ref{eq:posing}).
  }}
  \label{fig:qualitative}
  \vspace{-0.4cm}
\end{figure*}










==> figure_supp_internet.tex <==
\begin{figure*}[t!]
  \vspace{-0.1cm}
  \includegraphics[width=\linewidth, trim={0.1cm 0.1cm 0cm 0}, clip = true]{figures/internet_supp.png}
        \put(-485,4){{{Input image}}}
        \put(-338,4){{{CRMH~\cite{jiang2020_multiperson}}}}
        \put(-115,4){{{Ours}}}
  \vspace{0.2cm}
  \caption{\small{\textbf{Qualitative results}. We visualize the results of our method from different viewpoints: front (green background), top (blue background), and side (red background) views. We compare the results with CRMH~\cite{jiang2020_multiperson} and improve depth order and overall scene coherence. Note that CRMH does not estimate a plane. We add the same plane estimated by our method for the visualization purposes.
%   We have improved results in terms of depth order and overall scene coherence. Notice people's depth order and sizes.
  %(see Eq.~\ref{eq:posing}).
  }}
  \label{fig:qualitative}
  \vspace{-0.4cm}
\end{figure*}






==> figure_supp_mupots.tex <==
\begin{figure*}[t!]
  \vspace{-0.1cm}
  \includegraphics[width=\linewidth, trim={0.1cm 0.1cm 0cm 0}, clip = true]{figures/mupots_supp.png}
        \put(-485,4){{{Input image}}}
        \put(-338,4){{{CRMH~\cite{jiang2020_multiperson}}}}
        \put(-115,4){{{Ours}}}
  \vspace{0.2cm}
  \caption{\small{\textbf{Qualitative results}. We visualize the results of our method from different viewpoints: front (green background), top (blue background), and side (red background) views. We compare the results with CRMH~\cite{jiang2020_multiperson} and improve depth order and overall scene coherence. Note that CRMH does not estimate a plane. We add the same plane estimated by our method for the visualization purposes.
%   We have improved results in terms of depth order and overall scene coherence. Notice people's depth order and sizes.
  %(see Eq.~\ref{eq:posing}).
  }}
  \label{fig:qualitative}
  \vspace{-0.4cm}
\end{figure*}






==> section_05_implementation.tex <==
\section{Implementation}\label{sec:implementation}
We next describe the main implementation details. Further information is provided in the code that will be made publicly available.

We jointly optimize for both translation and scale using the ADAM optimizer~\cite{adam} with learning rate 1e-2 for either 600 iterations. As for reference 2D keypoints, we use the 3D reprojected joints obtained from the initial SMPL estimations from either CRMH~\cite{jiang2020_multiperson} or FrankMocap\cite{totalCapture_frank}. We present experiments with these two initializations in Sec.~\ref{sec:experiments}, however, given the nature of our method, any other initialization can be used. 
We use semantic segmentation from Detectron2~\cite{detectron2} for our baseline and use MiDas v3.~\cite{midas_ranftl2021} as depth estimator. For all cases we use a fixed focal lenght of $f=1000$.


As for the scale parameter used to transform the depth map from relative values to absolute ones, we use the value 6.0 for both Mupots and 3DPW because...\nico{aqui se necesita explicacion, all our reported experiments use a scale of 6.0, so easier to explain}.
